Straggler Mitigation at Scale

Runtime performance variability at the servers has been a major issue, hindering the predictable and scalable performance in modern distributed systems. Executing requests or jobs redundantly over multiple servers has been shown to be effective for mitigating variability, both in theory and practice. Systems that employ redundancy has drawn significant attention, and numerous papers have analyzed the pain and gain of redundancy under various service models and assumptions on the runtime variability. This paper presents a cost (pain) vs. latency (gain) analysis of executing jobs of many tasks by employing replicated or erasure coded redundancy. Tail heaviness of service time variability is decisive on the pain and gain of redundancy and we quantify its effect by deriving expressions for the cost and latency. Specifically, we try to answer four questions: 1) How do replicated and coded redundancy compare in the cost vs. latency tradeoff? 2) Can we introduce redundancy after waiting some time and expect to reduce the cost? 3) Can relaunching the tasks that appear to be straggling after some time help to reduce cost and/or latency? 4) Is it effective to use redundancy and relaunching together? We validate the answers we found for each of the questions via simulations that use empirical distributions extracted from a Google cluster data.

==> proofs/Thm-1_proof_deprecated.tex <==
% Includes the derivations that are deemed to be overly complex and replaced by their simpler counterparts
% ###  Pr{T > t}  ### %
  \vspace{0.2em}
  \noindent
  \textbf{Distribution of job execution time, \eqref{eqn:eq_k_cd_Exp_tail}.}
  Using the law of total probability, we have
  \begin{equation}
  \begin{split}
    \Pr\{T > t\} &= \Pr\{T > t \mid T \leq \Delta\}\Pr\{T \leq \Delta\} \\
	&+ \Pr\{T > t \mid T > \Delta\}\Pr\{T > \Delta\},
  \end{split}
  \label{eqn:eq_k_cd_Exp__tail_condsum}
  \end{equation}
  where the left hand side is given as
  \begin{longaligned}[\label{eqn:eq_k_cd_Exp__tail_condsum_lhs}]
    \Pr\{& T > t \mid T \leq \Delta\}\Pr\{T \leq \Delta\} \\
    &= \Pr\{X_{k:k} > t \mid X_{k:k} \leq \Delta\}\Pr\{X_{k:k} \leq \Delta\} \\
    &= \mathbbm{1}(t \leq \Delta)\left(\Pr\{X_{k:k} \leq \Delta\} - \Pr\{X_{k:k} \leq t\}\right) \\
    &= \mathbbm{1}(t \leq \Delta)\left((1-e^{-\mu\Delta})^k - (1-e^{-\mu t})^k \right). \longalignedtag
  \end{longaligned}
  where we used the identities $T \mid T \leq \Delta \sim X_{k:k}$ and $\Pr\{X_{k:k} \leq t\} = \Pr\{X \leq t\}^k$.
  Let $R$ be the number of tasks completed before time $\Delta$, hence $R \sim \mathrm{Bin}(k, q)$ with $q = 1 - e^{-\mu\Delta}$.
  Right hand side of the sum in \eqref{eqn:eq_k_cd_Exp__tail_condsum} is given as
  \begin{longaligned}[\label{eqn:eq_k_cd_Exp__tail_condsum_rhs}]
    \Pr\{& T > t \mid T > \Delta\}\Pr\{T > \Delta\} \\
    &= \Pr\{T > t \mid R < k\}\Pr\{R < k\} \\
    &= \sum_{r=0}^{k-1} \Pr\{T > t \mid R=r\}\Pr\{R=r\} \\
    &\stackrel{(a)}{=} \sum_{r=0}^{k-1} \left(1 - \Pr\{\tilde{X}_{k-r:k-r} + \Delta \leq t\}\right)\Pr\{R=r\} \\
    &= (1 - q^k) - \left(\E\left[\Pr\{\tilde{X} \leq t-\Delta\}^{k-R}\right] - q^k\right) \\
    &\stackrel{(c)}{=} 1 - \left(q + (1-q)\mathbbm{1}(t > \Delta)\left(1-e^{-(c+1)\mu(t-\Delta)}\right)\right)^k. \longalignedtag
  \end{longaligned}
  Equality $(a)$ results from the following observation. For each of the $k-r$ tasks remaining at time $\Delta$, $c$ fresh replicas are launched. \emph{Residual} lifetime of each of these remaining tasks is $\tilde{X} \sim \mathrm{Exp}((c+1)\mu)$ because each task completes as soon as the fastest of its $c+1$ copies completes and due to the memoryless property of the exponential execution times, each copy takes $\mathrm{Exp}(\mu)$ to complete, and minimum of $c+1$ i.i.d. $\mathrm{Exp}(\mu)$'s is distributed as $\mathrm{Exp}((c+1)\mu)$.
  Job is completed when all remaining tasks complete, so the residual lifetime of the job after time $\Delta$ is given as $\tilde{X}_{k-r:k-r}$.
  Equality $(c)$ results from the probability generating function for $R$.
  Putting \eqref{eqn:eq_k_cd_Exp__tail_condsum_lhs} and \eqref{eqn:eq_k_cd_Exp__tail_condsum_rhs} together gives \eqref{eqn:eq_k_cd_Exp_tail}.
% ### E[C] ### %
By the law of total expectation,
  \begin{longaligned}[\label{eqn:eq_k_cd_Exp__EC_condsum1}]
    E[C] &= E[C|T \leq \Delta]Pr\{T \leq \Delta\} + E[C|T > \Delta]Pr\{T > \Delta\} \\
    &= E[C|X_{k:k} \leq \Delta]Pr\{X_{k:k} \leq \Delta\} \\
    &\quad + E[C|X_{k:k} > \Delta]Pr\{X_{k:k} > \Delta\}. \longalignedtag
  \end{longaligned}
  Let $C_0$ represent the cost when no redundancy is employed, then its expected value is found as
  \begin{longaligned}[\label{eqn:eq_k_cd_Exp__EC_condsum2}]
    E[C_0] &= E[C_0|T \leq \Delta]Pr\{T \leq \Delta\} + E[C_0|T > \Delta]Pr\{T > \Delta\} \\
    &= E[C_0|X_{k:k} \leq \Delta]Pr\{X_{k:k} \leq \Delta\} \\
    &\quad + E[C_0|X_{k:k} > \Delta]Pr\{X_{k:k} > \Delta\}. \longalignedtag
  \end{longaligned}
  Observe that given a job completes before $\Delta$, the cost is the same either redundancy is employed or not. Then we take the difference
  \begin{longaligned}[\label{eqn:eq_k_cd_Exp__EC_condsum3}]
    E[C] - E[C_0] &= E[C|X_{k:k} > \Delta]Pr\{X_{k:k} > \Delta\} \\
    &\quad - E[C_0|X_{k:k} > \Delta]Pr\{X_{k:k} > \Delta\}. \longalignedtag
  \end{longaligned}
  Denoting the number of tasks completed before $\Delta$ as $R \sim \textit{Bin}(k,q)$ where $q = 1-e^{-\mu\Delta}$, left hand side of this difference is
  \begin{equation}
    E[C | X_{k:k} > \Delta]Pr\{X_{k:k} > \Delta\} = \sum_{r=0}^{k-1} E[C|R=r]Pr\{R=r\}.
  \label{eqn:eq_k_cd_Exp__EC_condsum3_lhs}
  \end{equation}
  Observing that given $r < k$ tasks completed before $\Delta$, the total cost is equal to the total lifetime of the initial tasks as $\sum_{i=1}^r E[X_i|X_i \leq \Delta] + \sum_{i=1}^{k-r} E[X_i|X_i > \Delta]$ and the total lifetime of the replica tasks as $c\sum_{i=1}^{k-r} E[X_i]$. In summary
  \begin{longaligned}
    E[C|R=r] &= \sum_{i=1}^r E[X_i|X_i \leq \Delta] \\
    &+ \sum_{i=1}^{k-r} E[X_i|X_i > \Delta] + c\sum_{i=1}^{k-r} E[X_i].
  \end{longaligned}
  
  In the same way, the right hand side of the difference in \eqref{eqn:eq_k_cd_Exp__EC_condsum3} is
  \begin{longaligned}[\label{eqn:eq_k_cd_Exp__EC_condsum3_rhs}]
    & E[C_0 | X_{k:k} > \Delta]Pr\{X_{k:k} > \Delta\} = \sum_{r=0}^{k-1} E[C_0|R=r]Pr\{R=r\} \\
    &\stackrel{(a)}{=} \sum_{r=0}^{k-1} \Bigl(\sum_{i=1}^r E[X_i|X_i \leq \Delta] + \sum_{i=1}^{k-r} E[X_i|X_i > \Delta]\Bigr)\Pr\{R=r\}. \longalignedtag
  \end{longaligned}
  putting \eqref{eqn:eq_k_cd_Exp__EC_condsum3_lhs} and \eqref{eqn:eq_k_cd_Exp__EC_condsum3_rhs} in \eqref{eqn:eq_k_cd_Exp__EC_condsum3}
  \begin{longaligned}[\label{eqn:eq_k_cd_Exp__EC_condsum}]
    E[C] - E[C_0] &= \sum_{r=0}^{k-1} \Bigl(c\sum_{i=1}^{k-r} E[X_i]\Bigr)\Pr\{R=r\} \\
    &= c\Bigl(\sum_{r=0}^{k-1} \frac{k-r}{\mu} \Pr\{R=r\}\Bigr) \\
    &= c\Bigl(\frac{k}{\mu}(1-q^k) - \frac{k}{\mu}(q-q^k)\Bigr) = c\frac{k}{\mu}(1-q). \longalignedtag
  \end{longaligned}
  We have $E[C_0] = E[\sum_{i=1}^k X_{k:i}] = k/\mu$, and substituting which in \eqref{eqn:eq_k_cd_Exp__EC_condsum} gives $E[C]$ as stated in \eqref{eqn:eq_k_cd_Exp_EC}.
  
% ### E[C^c] ### %
By the law of total expectation
  \begin{longaligned}[\label{eqn:eq_k_cd_Exp__ECwcancel_condsum1}]
    E[C^c] &= E[C^c|T \leq \Delta]Pr\{T \leq \Delta\} \\
    &\quad + E[C^c|T > \Delta]Pr\{T > \Delta\} \\
    &= E[C^c|X_{k:k} \leq \Delta]Pr\{X_{k:k} \leq \Delta\} \\
    &\quad + E[C^c|X_{k:k} > \Delta]Pr\{X_{k:k} > \Delta\}. \longalignedtag
  \end{longaligned}
  By \eqref{eqn:eq_k_cd_Exp__ECwcancel_condsum1} and \eqref{eqn:eq_k_cd_Exp__EC_condsum1}, difference between the cost with and without task cancellation is given as
  \begin{longaligned}[\label{eqn:eq_k_cd_Exp__ECwcancel_minus_EC}]
    E[C^c] - E[C] &= E[C^c|X_{k:k} > \Delta]Pr\{X_{k:k} > \Delta\} \\
    &- E[C|X_{k:k} > \Delta]Pr\{X_{k:k} > \Delta\}. \longalignedtag
  \end{longaligned}
  The right hand side of this difference
  \begin{longaligned}[\label{eqn:eq_k_cd_Exp__ECwcancel_condsum2}]
    & E[C^c | X_{k:k} > \Delta]Pr\{X_{k:k} > \Delta\} \\
    &\stackrel{(a)}{=} \sum_{r=0}^{k-1} \Bigl(\sum_{i=1}^r E[X_i|X_i \leq \Delta] + \sum_{i=1}^{k-r} (\Delta + cE[\tilde{X_i}])\Bigr)\Pr\{R=r\} \\
    &\stackrel{(b)}{=} \sum_{r=0}^{k-1} \Bigl(\sum_{i=1}^r E[X_i|X_i \leq \Delta] + \sum_{i=1}^{k-r} E[X_i|X_i > \Delta]\Bigr)\Pr\{R=r\}. \longalignedtag
  \end{longaligned}
  where $(a)$ is by observing that the total cost added by the $k-r$ tasks that took beyond time $\Delta$ and the replicas of each is given as $\sum_{i=1}^{k-r} \Delta + cE[\tilde{X_i}]$ in which $\tilde{X_i} \sim \textit{Exp}(c\mu)$ using the memoryless property. $(b)$ is by noticing that $\Delta + E[\tilde{X_i}] = \Delta + 1/\mu = E[X_i|X_i > \Delta]$. Substituting \eqref{eqn:eq_k_cd_Exp__EC_condsum3_lhs} and \eqref{eqn:eq_k_cd_Exp__ECwcancel_condsum2} in \eqref{eqn:eq_k_cd_Exp__ECwcancel_minus_EC}, we get
  \begin{longaligned}[\label{eqn:eq_k_cd_Exp__ECwcancel_condsum3}]
    E[C^c] - E[C] &= -\sum_{r=0}^{k-1} \Bigl(c\sum_{i=1}^{k-r} E[X_i]\Bigr)\Pr\{R=r\} \\
    &= -\frac{k}{\mu}c(1-q). \longalignedtag
  \end{longaligned}
  which together with the expression we previously derived for cost $E[C]$ without task cancellation gives the expression of the cost $E[C^c]$ with task cancellation as in \eqref{eqn:eq_k_cd_Exp_EC}.

==> proofs/Thm-2_proof_deprecated.tex <==
% ### C^c ### %
% ### E[C^c] ### %
  \vspace{0.2em}
  \noindent
  \textbf{Cost with task cancellation, \eqref{eqn:eq_k_cd_SExp_ECwcancel}.}
  Each task takes at least $s/k$ time to complete.
  Firstly, suppose $\Delta \leq s/k$, then replicas will be launched for each task since a task can not complete before time $\Delta$.
  We next inspect the lifetime of a single task.
  Let us refer to job launch time as $0$. Then, in time interval $[0, \Delta]$, only task's original copy runs.
  At time $\Delta$, $c$ replicas are launched for the task, so in $[\Delta, \Delta + s/k]$ task has total $c+1$ copies running.
  At time $s/k$, deterministic portion of original copy's execution time will be over and its residual lifetime will be determined by an $\mathrm{Exp}(\mu)$ timer, while each replica will take until time $s/k + \Delta$ to finish the deterministic portion of their lifetime.
  Thus, original copy can complete before time $s/k + \Delta$, then all task copies would get cancelled, or it would last until time $s/k + \Delta$, then all $c+1$ copies will start a timer at time $s/k + \Delta$ and job will complete as soon as the fastest copy completes.
  Therefore, task's contribution to cost will be $\Delta + (c+1)(s/k - \Delta)$ until time $s/k$,
  and afterwards it will be 
  \begin{equation*}
  \begin{split}
    & \Pr\{\tilde{X} \leq \Delta\}(c+1)\E[\tilde{X} \mid \tilde{X} \leq \Delta] \\
    &\quad + \Pr\{\tilde{X} > \Delta\}\left((c+1)\Delta + (c+1)\frac{1}{(c+1)\mu} \right)
  \end{split}
  \end{equation*}
  for $\tilde{X} \sim \mathrm{Exp}(\mu)$. Cost contributions before or after time $s/k$ adds up to
  \[ (c+1)\frac{s}{k} + \frac{c+1}{\mu} - c\Delta - \frac{c}{\mu}e^{-\mu\Delta}. \]
  Job consists of $k$ tasks, thus, multiplying the expression above by $k$ yields the case $\Delta \leq s/k$ in \eqref{eqn:eq_k_cd_SExp_ECwcancel}.
  
  Secondly, suppose $\Delta > s/k$,
  
  % ### C ### %
  \vspace{0.2em}
  \noindent
  \textbf{Cost without task cancellation, \eqref{eqn:eq_k_cd_SExp_EC}.}
  By the total law of expectation,
  \[ \E[C] = \sum_{r=0}^k \E[C \mid R=r]\Pr\{R=r\}. \]
  Suppose $R=r$. Then, sum of the lifetimes of $r$ tasks that finish before time $\Delta$ is given as $\sum_{r=0}^k \left(\sum_{i=1}^r \E[X_i \mid X_i \leq \Delta]\right)$, and sum of the lifetimes of those that finish after time $\Delta$ and their replicas is given as $\sum_{i=1}^{k-r} \E[X_i \mid X_i > \Delta] + c\E[X_i]$.
  Thus, we have
  \begin{longaligned}
    \E[C] &= \E\left[R \E[X \mid X \leq \Delta] \right] \\
      &\quad + \E\left[(k-R)\left(\E[X \mid X > \Delta] + c\E[X]\right)\right] \\
    &= kq\E[X \mid X \leq \Delta] \\
      &\quad + k(1-q)\left(\E[X \mid X > \Delta] + c\E[X]\right) \\
    &= k\left(\E[X] + c(1-q)\E[X]\right) = k\left(c(1-q) + 1\right)\E[X].
  \end{longaligned}
  Substituting $\E[X] = s/k + 1/\mu$ above yields \eqref{eqn:eq_k_cd_SExp_EC}.

==> proofs/Thm-3_proof_deprecated.tex <==
\vspace{0.2em}
  \noindent
  \textbf{Cost without task cancellation, $\E[C]$ in \eqref{eqn:eq_k_nd_Exp_EC}.}
  Let us work with a generalized coded redundancy system where $l-k$ coded tasks are launched together with $k$ initial tasks at time $0$, then if the job still runs at time $\Delta$, $n-l$ more coded tasks are introduced into the execution.
  By the law of total expectation
  \begin{longaligned}[\label{eqn:eq_k_nd_Exp__EC_condsum}]
    \E[C] &= \E[C \mid T \leq \Delta]\Pr\{T \leq \Delta\} \\
    &\quad + \E[C \mid T > \Delta]\Pr\{T > \Delta\}. \longalignedtag
  \end{longaligned}
  Left hand side of the sum above is
  \begin{longaligned}[\label{eqn:eq_k_nd_Exp__EC_condsum_lhs_1}]
    & \E[C \mid T \leq \Delta]\Pr\{T \leq \Delta\} = \E[C \mid R \geq k]\Pr\{R \geq k\} \\
    &= \sum_{r=k}^l \E[C \mid R=r]\Pr\{R=r\} \\
    &\stackrel{(a)}{=} \sum_{r=k}^l \Big(\sum_{i=1}^r \E[X_i \mid X_i \leq \Delta] \\
      &\quad\quad\quad\quad + \sum_{i=1}^{l-r} \E[X_i \mid X_i > \Delta]\Bigr) \Pr\{R=r\} \\
    &\stackrel{(b)}{=} \sum_{r=k}^l r\left(\frac{1}{\mu}-\Delta\frac{1-q}{q}\right) + (l-r)\left(\frac{1}{\mu}+\Delta\right) \Pr\{R=r\} \\
    &= \left(\frac{l}{\mu}+l\Delta\right)\Pr\{k \leq R \leq l\} - \frac{\Delta}{q}\sum_{r=k}^l r\Pr\{R=r\}. \longalignedtag
  \end{longaligned}
  Equality $(a)$ comes from noticing that the cost given $r$ task completions before $\Delta$ ($\E[C \mid R=r]$) is the sum of the lifetimes of $r$ tasks that complete before $\Delta$ and the lifetimes of the $l-r$ tasks that finish after $\Delta$. Equality $(b)$ is by substituting $\E[X_i \mid X_i \leq \Delta] = 1/\mu-\Delta(1-q)/q$ and $\E[X_i \mid X_i > \Delta] = 1/\mu+\Delta$ for $X_i \sim \mathrm{Exp}(\mu)$. One can write
  \begin{longaligned}
    \Pr\{k \leq & R \leq l\} = 1 - \Pr\{R < k\} \\
    &= 1 - I(1-q;l-k+1,k) = I(q;k,l-k+1).
  \end{longaligned}
  and
  \begin{longaligned}
    \sum_{r=k}^l r\Pr\{R=r\} &= \sum_{r=k}^l r\binom{l}{r} q^r (1-q)^{l-r} \\
    &\stackrel{(a)}{=} \sum_{r=k}^l l\binom{l-1}{r-1} q^r (1-q)^{l-r} \\
    &\stackrel{(b)}{=} l\sum_{r^{\prime}=k-1}^{l-1} \binom{l-1}{r^{\prime}} q^{r^{\prime}+1} (1-q)^{l-r^{\prime}-1} \\
    &= lq(1 - \sum_{r^{\prime}=0}^{k-2} \binom{l-1}{r^{\prime}} q^{r^{\prime}} (1-q)^{l-1-r^{\prime}}) \\
    &= lq\left(1 - I(1-q;l-k+1,k-1)\right) \\
    &= lq\;I(q;k-1,l-k+1).
  \end{longaligned}
  Equality $(a)$ is by the identity $r\binom{l}{r} = l\binom{l-1}{r-1}$, $(b)$ is by introducing the variable $r^{\prime} = r-1$.
  Substituting these back in \eqref{eqn:eq_k_nd_Exp__EC_condsum_lhs_1} gives
  \begin{equation}
  \begin{split}
    \E[C \mid T \leq \Delta]\Pr\{T \leq \Delta\} &= l(1/\mu+\Delta)I(q;k,l-k+1) \\
    &\quad - l\Delta I(q;k-1,l-k+1).
  \end{split}
  \label{eqn:eq_k_nd_Exp__EC_condsum_lhs}
  \end{equation}
  
  Right hand side of the sum in \eqref{eqn:eq_k_nd_Exp__EC_condsum} is
  \begin{longaligned}[\label{eqn:eq_k_nd_Exp__EC_condsum_rhs_1}]
    & \E[C \mid T > \Delta]\Pr\{T > \Delta\} = \E[C \mid R < k]\Pr\{R < k\} \\
    &= \sum_{r=0}^{k-1} \E[C \mid R=r]\Pr\{R=r\} \\
    &\stackrel{(a)}{=} \sum_{r=0}^{k-1} \E\left[\sum_{i=1}^l X_{l:i} + \sum_{i=1}^{n-l} X_{n-l:i} \mid R=r\right]\Pr\{R=r\} \\
    &= \sum_{r=0}^{k-1} \Biggl(\E\left[\sum_{i=1}^l X_{l:i} \mid R=r\right] \\
      &\qquad\qquad + \E\left[\sum_{i=1}^{n-l} X_{n-l:i} \mid R=r\right]\Biggr)\Pr\{R=r\} \\
    &\stackrel{(b)}{=} \sum_{r=0}^{k-1} \Biggl(\sum_{i=1}^r \E[X_i \mid X_i \leq \Delta] \\
      &\quad\quad\quad + \sum_{i=1}^{l-r} \E[X_i \mid X_i > \Delta] + \frac{n-l}{\mu}\Biggr)\Pr\{R=r\} \\
    &= \sum_{r=0}^{k-1} \biggl(r\left(\frac{1}{\mu}-\Delta\frac{1-q}{q}\right) \\
      &\qquad\qquad + (l-r)\left(\frac{1}{\mu}+\Delta\right) + \frac{n-l}{\mu}\biggr)\Pr\{R=r\} \\
    &= \sum_{r=0}^{k-1} \left(\frac{n}{\mu} + \Delta\left(l-\frac{r}{q}\right)\right)\Pr\{R=r\} \\
    &= \left(\frac{n}{\mu}+l\Delta\right)\Pr\{R < k\} - \frac{\Delta}{q}\sum_{r=0}^{k-1} r\Pr\{R=r\}. \longalignedtag
  \end{longaligned}
  Equality $(a)$ is by observing that the cost given that the job did not complete before $\Delta$ is the sum of the lifetimes of all the initial $l$ tasks and later added $n-l$ redundant tasks. Equality $(b)$ comes from two observations. Firstly,
  \[ \E\left[\sum_{i=1}^{n-l} X_{n-l:i} \mid R=r\right] = \E\left[\sum_{i=1}^{n-l} X_{n-l:i}\right] \]
  because the execution time of redundant tasks are independent of the number of tasks completed before $\Delta$, so $\E\left[\sum_{i=1}^{n-l} X_{n-l:i}\right] = (n-l)/\mu$.
  Secondly, sum of the lifetimes of the initial tasks given $R=r$ is the sum of the lifetimes of the tasks that complete before $\Delta$ plus the sum of the lifetimes of the tasks that complete after $\Delta$.
  One can write $\Pr\{R < k\} = I(1-q;l-k+1,k)$ and
  \begin{longaligned}
    \sum_{r=0}^{k-1} r\Pr\{R=r\} &= \sum_{r=0}^{k-1} r\binom{l}{r} q^r (1-q)^{l-r} \\
    &\stackrel{(a)}{=} l\sum_{r=1}^{k-1} \binom{l-1}{r-1} q^r (1-q)^{l-r} \\
    &\stackrel{(b)}{=} lq\sum_{r^{\prime}=0}^{k-2} \binom{l-1}{r^{\prime}} q^{r^{\prime}} (1-q)^{l-1-r^{\prime}} \\
    &= lqI(1-q;l-k+1,k-1).
  \end{longaligned}
  Equality $(a)$ comes from the identity $r\binom{l}{r} = l\binom{l-1}{r-1}$, and $(b)$ by introducing $r^{\prime} = r-1$.
  Substituting these back in \eqref{eqn:eq_k_nd_Exp__EC_condsum_rhs_1} gives
  \begin{equation}
  \begin{split}
    \E[C \mid T > \Delta]\Pr\{T > \Delta\} &= \left(\frac{n}{\mu}+l\Delta\right)I(1-q;l-k+1,k) \\
    &\quad - l\Delta I(1-q;l-k+1,k-1).
  \end{split}
  \label{eqn:eq_k_nd_Exp__EC_condsum_rhs}
  \end{equation}
  Finally, substituting \eqref{eqn:eq_k_nd_Exp__EC_condsum_lhs} and \eqref{eqn:eq_k_nd_Exp__EC_condsum_rhs} in \eqref{eqn:eq_k_nd_Exp__EC_condsum} gives
  \begin{longaligned}
    & \E[C] = \frac{l}{\mu}I(q;k,l-k+1) + \frac{n}{\mu}I(1-q;l-k+1,k) \\
    &\quad + l\Delta\left[I(q;k,l-k+1) + I(1-q;l-k+1,k)\right] \\
    &\quad - l\Delta\left(I(q;k-1,l-k+1) - I(1-q;l-k+1,k-1)\right) \\
    &= \frac{l}{\mu}I(q;k,l-k+1) + \frac{n}{\mu}\left(1-I(q;k,l-k+1)\right).
%     = l(1/\mu+\Delta)I(q;k,l-k+1) \\
%     &\quad - l\Delta I(q;k-1,l-k+1) \\
%     &\quad + (n/\mu+l\Delta)I(1-q;l-k+1,k) \\
%     &\quad - l\Delta I(1-q;l-k+1,k-1) \\
  \end{longaligned}
  Setting $l = k$ in which gives the cost expression in \eqref{eqn:eq_k_nd_Exp_EC}.
  
  % ### E[C^c] ### %
  \vspace{0.2em}
  \noindent
  \textbf{Cost with task cancellation, $\E[C^c]$ in \eqref{eqn:eq_k_nd_Exp_EC}.}
  Again we consider the generalized coded redundancy system that we introduced above in order to derive $\E[C]$.
  By the law of total expectation,
  \begin{longaligned}[\label{eqn:eq_k_nd_Exp__ECwcancel_condsum_rhs}]
    \E[C^c] &= \E[C^c \mid T \leq \Delta]\Pr\{T \leq \Delta\} \\
    &\quad + \E[C^c \mid T > \Delta]\Pr\{T > \Delta\} \\
    &\stackrel{(a)}{=} \E\left[C-\frac{l-k}{\mu} \mid T \leq \Delta\right]\Pr\{T \leq \Delta\} \\
    &\quad + \E\left[C-\frac{n-k}{\mu} \mid T > \Delta\right]\Pr\{T > \Delta\} \\
    &= \E[C] - \frac{l-k}{\mu}\Pr\{R < k\} - \frac{l-k}{\mu}\Pr\{R \geq k\} \\
    &= \E[C] + \frac{k}{\mu} - \E[C] = \frac{k}{\mu}. \longalignedtag
  \end{longaligned}
  Equality $(a)$ is by noticing that the cost with task cancellation can be found by subtracting total residual lifetime of the tasks that continue after job completion from the cost without task cancellation. Without task cancellation, $l-k$ tasks remain after job completion if the job completes before $\Delta$, and $n-k$ tasks remain otherwise. Then, using the memoryless property of exponential, sum of the expected residual lifetime of the remaining tasks after job completion is found as $(l-k)/\mu$ if the job completes before $\Delta$ and as $(n-k)/\mu$ otherwise.
  Setting $l=k$ in \eqref{eqn:eq_k_nd_Exp__ECwcancel_condsum_rhs} yields $\E[C^c]$ as stated in \eqref{eqn:eq_k_nd_Exp_EC}.

==> proofs/proof_of_k_cd_wrelaunch_ET__EC.tex <==
\begin{proof}
  % ### E[T] ### %
  First, we derive the expression for latency. Let $E[T_{wo}]$ be the latency of job execution when straggler relaunch is performed at time $\Delta$ with no redundancy employed. Exact expression for $E[T_{wo}]$ is given in \eqref{eqn:eq_k_wrelaunch_tail__ET}. Using the law of total expectation
  \begin{longaligned}
    E[T_{wo}] &= E[T_{wo}|R=k]Pr\{R=k\} \\
    &\quad + \sum_{r=0}^{k-1} E[T_{wo}|R=r]Pr\{R=r\} \\
    &= E[X_{k:k}|R=k]Pr\{R=k\} \\
    &\quad + \sum_{r=0}^{k-1} E[\Delta + X_{k-r:k-r}]Pr\{R=r\}.
  \end{longaligned}
  Repeating the same for the latency of employing replicated redundancy together with straggler relaunch at time $\Delta$
  \begin{longaligned}
    E[T] &= E[T|R=k]Pr\{R=k\} + \sum_{r=0}^{k-1} E[T|R=r]Pr\{R=r\} \\
    &= E[X_{k:k}|R=k]Pr\{R=k\} \\
    &\quad + \sum_{r=0}^{k-1} E\bigl[\Delta + (X_{(c+1):1})_{k-r:k-r}\bigr]Pr\{R=r\}.
  \end{longaligned}
  where $X_{(c+1):1} \sim \textit{Pareto}(\lambda, (c+1)\alpha)$. Taking the difference between these two
  \begin{longaligned}
    & E[T] - E[T_{wo}] \\
    &= \sum_{r=0}^{k-1} E[(X_{(c+1):1})_{k-r:k-r} - X_{k-r:k-r}] Pr\{R=r\} \\
    &= E\bigl[E[(X_{(c+1):1})_{k-R:k-R} - X_{k-R:k-R}|R]\bigr] \\
    &= \lambda\Gamma(1-1/(c+1)\alpha)E\Bigl[\frac{\Gamma(k-R+1)}{\Gamma(k-R+1-1/(c+1)\alpha)}\Bigr] \\
    &\quad - \lambda\Gamma(1-1/\alpha)E\Bigl[\frac{\Gamma(k-R+1)}{\Gamma(k-R+1-1/\alpha)}\Bigr] \\
    &= \lambda\frac{\Gamma(1-1/(c+1)\alpha)}{\Gamma(-1/(c+1)\alpha)}E\Bigl[\frac{\Gamma(k-R+1)\Gamma(-1/(c+1)\alpha)}{\Gamma(k-R+1-1/(c+1)\alpha)}\Bigr] \\
    &\quad - \lambda\frac{\Gamma(1-1/\alpha)}{\Gamma(-1/\alpha)}E\Bigl[\frac{\Gamma(k-R+1)\Gamma(-1/\alpha)}{\Gamma(k-R+1-1/\alpha)}\Bigr] \\
    &= \lambda\frac{\Gamma(1-1/(c+1)\alpha)}{\Gamma(-1/(c+1)\alpha)}E[B(k-R+1, -1/(c+1)\alpha)] \\
    &\quad - \lambda\frac{\Gamma(1-1/\alpha)}{\Gamma(-1/\alpha)}E[B(k-R+1, -1/\alpha)] \\
    &\stackrel{(a)}{\approx} \lambda\frac{\Gamma(1-1/(c+1)\alpha)}{\Gamma(-1/(c+1)\alpha)}B(k-kq+1, -1/(c+1)\alpha) \\
    &\quad - \lambda\frac{\Gamma(1-1/\alpha)}{\Gamma(-1/\alpha)}B(k-kq+1, -1/\alpha).
  \end{longaligned}
  where $(a)$ is by Lemma \ref{lm_approx_bin_mean_of_harmonic__ibeta}.
  
  % ### E[C] ### %
  Next, we derive the cost without task cancellation. Let $R$ be the number of tasks completed before time $\Delta$, then $R \sim \textit{Bin}(k, q)$ where $q = \mathbbm{1}(\Delta > \lambda)(1 - (\lambda/\Delta)^{\alpha})$. Using iterated expectation
  \begin{longaligned}
    & E[C] = E\Bigl[E[C|R]\Bigr] \\
    &= E\Bigl[E\Bigl[\sum_{i=1}^R (X_i|X_i \leq \Delta) + (k-R)\Delta \\
    &\qquad\quad + \sum_{i=1}^{k-R} (c+1)X_{k-R:i} |R\Bigr]\Bigr] \\
    &= E\Bigl[R E[X_i|X_i \leq \Delta] + (k-R)\Delta \\
    &\qquad\quad + (c+1)(k-R)E[X]\Bigr] \\
    &= kqE[X_i|X_i \leq \Delta] + k(1-q)\Delta + k(c+1)(1-q)E[X] \\
    &\stackrel{(a)}{=} \frac{k\alpha}{(\alpha-1)}(\lambda - \Delta(1-q)) \\
    &\quad + k(1-q)\Delta + k(c+1)(1-q)\lambda\frac{\alpha}{\alpha-1}.
  \end{longaligned}
  where $(a)$ is by $E[X|X \leq \Delta] = \frac{\alpha}{q(\alpha-1)}(\lambda - \Delta(1-q))$ and $E[X] = \lambda\frac{\alpha}{\alpha-1}$.
  
  % ### E[C^c] ### %
  Next, we derive the cost with task cancellation. Using iterated expectation
  \begin{longaligned}
    & E[C^c] = E\Bigl[E[C^c|R]\Bigr] \\
    &= E\Bigl[E\Bigl[\sum_{i=1}^R (X_i|X_i \leq \Delta) + (k-R)\Delta \\
    &\qquad\quad + \sum_{i=1}^{k-R} (c+1)(X_{c+1:1})_{k-R:i} |R\Bigr]\Bigr] \\
    &= E\Bigl[R E[X|X \leq \Delta] + (k-R)\Delta + (c+1)(k-R)E[X_{c+1:1}]\Bigr] \\
    &= kqE[X|X \leq \Delta] + k(1-q)\Delta + k(c+1)(1-q)E[X_{c+1:1}] \\
    &\stackrel{(a)}{=} \frac{k\alpha}{(\alpha-1)}(\lambda - \Delta(1-q)) \\
    &\quad + k(1-q)\Delta + k(c+1)(1-q)\lambda\frac{(c+1)\alpha}{(c+1)\alpha-1}.
  \end{longaligned}
  where $(a)$ is by $E[X|X \leq \Delta] = \frac{\alpha}{q(\alpha-1)}(\lambda - \Delta(1-q))$ and $E[X_{c+1:1}] = \lambda\frac{(c+1)\alpha}{(c+1)\alpha-1}$.
\end{proof}


==> proofs/proof_of_k_nd_wrelaunch_ET__EC.tex <==
\begin{proof}
  % ### E[T] ### %
  Firstly, we derive the expression of latency. When $\Delta \leq \lambda$, all $k$ tasks that are initially launched at time $0$ will be relaunched together with $n-k$ new coded tasks at time $\Delta$, since no task can complete before time $\Delta \leq \lambda$. Equivalently, we think of the system performing the following: wait for $\Delta$, then launch $n$ tasks, among which any $k$ is sufficient for the job completion. Therefore, job completion time is simply $\Delta + E[X_{n:k}]$, then using the mean of Pareto order statistics gives the expression in \eqref{eqn:eq_k_nd_wrelaunch_ET} for $\Delta \leq \lambda$.
  
  When $\Delta > \lambda$, using the law of total expectation and denoting the number of tasks completed before time $\Delta$ as $R \sim \textit{Bin}(k, q)$ for $q = \mathbbm{1}(\Delta > \lambda)(1 - (\lambda/\Delta)^{\alpha})$, we have
  \begin{longaligned}[\label{eqn:eq_k_nd_wrelaunch_ET_totalexpec}]
    E[T] &= E[T|T \leq \Delta]Pr\{T \leq \Delta\} + E[T|T > \Delta]Pr\{T > \Delta\} \\
    &= E[X_{k:k}|R = k]Pr\{R = k\} \longalignedtag \\
    &\quad + E[\Delta + X_{n-R:k-R}|R < k]Pr\{R < k\}.
  \end{longaligned}
  
  Let $E[T_{wo}]$ be the latency when straggler relaunch is performed with no redundancy introduced. Exact expression of $E[T_{wo}]$ is given in \eqref{eqn:eq_k_wrelaunch_tail__ET}. Using the law of total expectation
  \begin{longaligned}[\label{eqn:eq_k_nd_wrelaunch_ET_totalexpec_2}]
    E[T_{wo}] &= E[T_{wo}|T_{wo} \leq \Delta]Pr\{T_{wo} \leq \Delta\} \\
    &\quad + E[T_{wo}|T_{wo} > \Delta]Pr\{T_{wo} > \Delta\} \\
    &= E[X_{k:k}|R = k]Pr\{R = k\} \longalignedtag \\
    &\quad + E[\Delta +	 X_{k-R:k-R}|R < k]Pr\{R < k\}.
  \end{longaligned}
  
  Taking the difference between \eqref{eqn:eq_k_nd_wrelaunch_ET_totalexpec} and \eqref{eqn:eq_k_nd_wrelaunch_ET_totalexpec_2}
  \begin{longaligned}[\label{eqn:eq_k_nd_wrelaunch_ET_diff}]
    & E[T] - E[T_{wo}] = \Bigl(E[X_{n-R:k-R}|R < k] \\
    &\qquad - E[X_{k-R:k-R}|R < k]\Bigr)Pr\{R < k\} \\
    &= \sum_{r=0}^{k-1} \Bigl(E[X_{n-r:k-r}] - E[X_{k-r:k-r}]\Bigr)Pr\{R=r\} \\
    &\stackrel{(a)}{=} \sum_{r=0}^{k-1} \Bigl(\lambda\frac{\Gamma(n-k+1-1/\alpha)}{(n-k)!}\frac{(n-r)!}{\Gamma(n-r+1-1/\alpha)} \\
    &\qquad - \lambda\Gamma(1-1/\alpha)\frac{(k-r)!}{\Gamma(k-r+1-1/\alpha)}\Bigr)Pr\{R=r\} \\
    &= \lambda\frac{\Gamma(n-k+1-1/\alpha)}{(n-k)!}E\Bigl[\frac{(n-R)!}{\Gamma(n-R+1-1/\alpha)}\Bigr] \longalignedtag \\
    &\quad - \lambda\Gamma(1-1/\alpha)E\Bigl[\frac{(k-R)!}{\Gamma(k-R+1-1/\alpha)}\Bigr]
  \end{longaligned}
  where $(a)$ is by using the mean of Pareto order statistics and observing that $E[X_{n-r:k-r}] - E[X_{k-r:k-r}] = 0$ for $r = k$. Then
  \begin{longaligned}
    E\Bigl[ & \frac{(k-R)!}{\Gamma(k-R+1-1/\alpha)}\Bigr] \\
    &= \sum_{r=0}^k \frac{(k-r)!}{(k-r-1/\alpha)!} \binom{k}{r} q^r(1-q)^{k-r} \\
    &= \frac{q^k}{\Gamma(1-1/\alpha)} + \sum_{r=0}^{k-1} \frac{k!}{(k-r-1/\alpha)!r!} q^r(1-q)^{k-r} \\
    &= \frac{q^k}{\Gamma(1-1/\alpha)} \\
    &\quad + \frac{k!}{\Gamma(k+1-1/\alpha)}\frac{\lambda}{\Delta} \sum_{r=0}^{k-1} \binom{k-1/\alpha}{r} q^r(1-q)^{k-r-1/\alpha} \\
    &= \frac{q^k}{\Gamma(1-1/\alpha)} + \frac{k!}{\Gamma(k+1-1/\alpha)}\frac{\lambda}{\Delta} I(1-q;1-1/\alpha,k).
  \end{longaligned}
  substituting which in \eqref{eqn:eq_k_nd_wrelaunch_ET_diff} gives
  \begin{longaligned}
    E[T] &- E[T_{wo}] \\
    &= \lambda\frac{\Gamma(n-k+1-1/\alpha)}{(n-k)!}E\Bigl[\frac{(n-R)!}{\Gamma(n-R+1-1/\alpha)}\Bigr] \\
    &\quad - \lambda\Gamma(1-1/\alpha)E\Bigl[\frac{(k-R)!}{\Gamma(k-R+1-1/\alpha)}\Bigr] \\
    &= \lambda\frac{\Gamma(n-k+1-1/\alpha)}{(n-k)!}E\Bigl[\frac{(n-R)!}{\Gamma(n-R+1-1/\alpha)}\Bigr] \\
    &\quad - \lambda q^k - k\frac{\lambda^2}{\Delta}\frac{\Gamma(1-1/\alpha)\Gamma(k)}{\Gamma(k+1-1/\alpha)}I(1-q;1-1/\alpha,k) \\
  &= \lambda\frac{\Gamma(n-k+1-1/\alpha)}{(n-k)!}E\Bigl[\frac{(n-R)!}{\Gamma(n-R+1-1/\alpha)}\Bigr] \\
    &\quad - \lambda q^k - k\frac{\lambda^2}{\Delta}B(1-1/\alpha,k)I(1-q;1-1/\alpha,k).
  \end{longaligned}
  Then, using the expression of $E[T_{wo}]$ that is given in \eqref{eqn:eq_k_wrelaunch_tail__ET}
  \begin{longaligned}[\label{eqn:eq_k_nd_wrelaunch_ET_almost}]
    & E[T] = \lambda\frac{\Gamma(n-k+1-1/\alpha)}{(n-k)!}E\Bigl[\frac{(n-R)!}{\Gamma(n-R+1-1/\alpha)}\Bigr] \\
    &\quad - \lambda q^k - k\frac{\lambda^2}{\Delta}B(1-1/\alpha,k)I(1-q;1-1/\alpha,k) + \Delta(1-q^k) \\
    &\quad + k\lambda B(1-1/\alpha,k)\Bigl(1 - (1-\frac{\lambda}{\Delta})I(1-q;1-1/\alpha,k)\Bigr) \\
    &= \lambda\frac{\Gamma(n-k+1-1/\alpha)}{(n-k)!}E\Bigl[\frac{(n-R)!}{\Gamma(n-R+1-1/\alpha)}\Bigr] \longalignedtag \\
    &\quad - \lambda q^k + \Delta(1-q^k) + k\lambda B(q;k,1-1/\alpha).
  \end{longaligned}
  Although the equality $B(x,y) = \Gamma(x)\Gamma(y)/\Gamma(x+y)$ can be shown with the integral evaluation of $B$ and $\Gamma$ functions only for $Re\{x\}, Re\{y\} > 0$, {\it analytic continuation} of these functions lets us do the following manipulation
  \begin{longaligned}
    & \frac{\Gamma(n-k+1-1/\alpha)}{(n-k)!}E\Bigl[\frac{(n-R)!}{\Gamma(n-R+1-1/\alpha)}\Bigr] \\
    &= \frac{\Gamma(n-k+1-1/\alpha)}{\Gamma(n-k+1)\Gamma(-1/\alpha)}E\Bigl[\frac{\Gamma(n-R+1)\Gamma(-1/\alpha)}{\Gamma(n-R+1-1/\alpha)}\Bigr] \\
    &= \frac{E[B(n-R+1,-1/\alpha)]}{B(n-k+1,-1/\alpha)} \stackrel{(a)}{\approx} \frac{B(n-kq+1,-1/\alpha)}{B(n-k+1,-1/\alpha)}.
  \end{longaligned}
  where $(a)$ is by Lemma \ref{lm_approx_bin_mean_of_harmonic__ibeta}. Substituting which in \eqref{eqn:eq_k_nd_wrelaunch_ET_almost} gives
  \begin{longaligned}
    E[T] &= \Delta(1-q^k) \\
    &\quad + \lambda\Bigl(\frac{B(n-kq+1,-1/\alpha)}{B(n-k+1,-1/\alpha)} + kB(q;k,1-1/\alpha) - q^k\Bigr).
  \end{longaligned}
  
  % ### E[C] ### %
  Next, we derive the cost without task cancellation. Using the law of total expectation
  \begin{longaligned}
    & E[C] = E[C|R=k]Pr\{R=k\} + \sum_{r=0}^{k-1} E[C|R=r]Pr\{R=r\} \\
    &= E\Bigl[\sum_{i=1}^k X_i|X_i \leq \Delta\Bigr]Pr\{R=k\} \\
    &\quad + \sum_{r=0}^{k-1} E\Bigl[\sum_{i=1}^r (X_i|X_i \leq \Delta) + (k-r)\Delta + \sum_{i=1}^{n-r} X_{n-r:i}\Bigr]Pr\{R=r\} \\
    &= \Bigl(\sum_{i=1}^k E[X|X \leq \Delta]\Bigr)Pr\{R=k\} \\
    &\quad + \sum_{r=0}^k E\Bigl[\sum_{i=1}^r (X_i|X_i \leq \Delta) + (k-r)\Delta + \sum_{i=1}^{n-r} X_{n-r:i}\Bigr]Pr\{R=r\} \\
    &\quad - E\Bigl[\sum_{i=1}^k (X_i|X_i \leq \Delta) + \sum_{i=1}^{n-k} X_{n-k:i}\Bigr]Pr\{R=k\} \\
    &= E\Bigl[E\Bigl[\sum_{i=1}^R (X_i|X_i \leq \Delta) + (k-R)\Delta + \sum_{i=1}^{n-R} X_{n-R:i}\Bigr]\Bigr] \\
    &\quad - E\Bigl[\sum_{i=1}^{n-k} X_{n-k:i}\Bigr]Pr\{R=k\} \\
    &= E\Bigl[R E[X|X \leq \Delta] + (k-R)\Delta + (n-R)E[X]\Bigr] \\
    &\quad - (n-k)E[X] q^k \\
    &= kqE[X|X \leq \Delta] + (k-kq)\Delta + (n-kq)E[X] \\
    &\quad - (n-k)E[X] q^k \\
    &\stackrel{(a)}{=} \frac{k\alpha}{\alpha-1}(\lambda - \Delta(1-q)) + (k-kq)\Delta + (n-kq)\frac{\lambda\alpha}{\alpha-1} \\
    &\quad - (n-k)q^k\frac{\lambda\alpha}{\alpha-1} \\
    &= \frac{\alpha}{\alpha-1}\Bigl(k\lambda - k\Delta(1-q) + n\lambda - k\lambda q - n\lambda q^k + k\lambda q^k\Bigr) \\
    &\quad + k(1-q)\Delta \\
    &= \frac{\alpha}{\alpha-1}\Bigl(k\lambda(1-q+q^k) + n\lambda(1-q^k)\Bigr) - \frac{k\Delta(1-q)}{\alpha-1}.
  \end{longaligned}
  where $(a)$ is by substituting the following
  \begin{longaligned}
    & E[X|X \leq \Delta] = \int_{\lambda}^{\Delta} xPr\{X=x|X \leq \Delta\}dx \\
    &= \int_{\lambda}^{\Delta} x \frac{Pr\{X=x\}}{Pr\{X \leq \Delta\}} dx = \frac{\alpha\lambda^{\alpha}}{q} \int_{\lambda}^{\Delta} x^{-\alpha}dx \\
    &= \frac{\lambda^{\alpha}}{q}\frac{\alpha}{\alpha-1}\Bigl(\lambda^{1-\alpha} - \Delta^{1-\alpha}\Bigr) = \frac{\alpha}{q(\alpha-1)}\Bigl(\lambda - \Delta(1-q)\Bigr).
  \end{longaligned}
  
  % ### E[C^c] ### %
  Next, we derive the expression for the cost with task cancellation. Using law of total expectation
  \begin{longaligned}[\label{eqn:eq_k_nd_wrelaunch_ECwcancel_lawoftotal}]
    & E[C^c] = E[C^c|R=k]Pr\{R=k\} \\
    &\quad + \sum_{r=0}^{k-1} E[C^c|R=r]Pr\{R=r\} \\
    &= E\Bigl[\sum_{i=1}^k X_i|X_i \leq \Delta\Bigr]Pr\{R=k\} + \sum_{r=0}^{k-1} E\Bigl[\sum_{i=1}^r (X_i|X_i \leq \Delta) \\
    &\quad + (k-r)\Delta + \sum_{i=1}^{k-r} X_{n-r:i} + (n-k)X_{n-r:k-r}\Bigr]Pr\{R=r\} \\
    &= \Bigl(\sum_{i=1}^k E[X|X \leq \Delta]\Bigr)Pr\{R=k\} + \sum_{r=0}^{k} E\Bigl[\sum_{i=1}^r (X_i|X_i \leq \Delta) \\
    &\quad + (k-r)\Delta + \sum_{i=1}^{k-r} X_{n-r:i} + (n-k)X_{n-r:k-r}\Bigr]Pr\{R=r\} \\
    &\quad - E\Bigl[\sum_{i=1}^k (X_i|X_i \leq \Delta) + (n-k)X_{n-k:0}\Bigr]Pr\{R=k\} \\
    &= E\Bigl[E\Bigl[\sum_{i=1}^R (X_i|X_i \leq \Delta) + (k-R)\Delta + \sum_{i=1}^{k-R} X_{n-R:i} \\
    &\quad + (n-k)X_{n-R:k-R} |R\Bigr]\Bigr] - \lambda(n-k)q^k \\
    &= kqE[X|X \leq \Delta] + k(1-q)\Delta \\
    &\quad + E\Bigl[\sum_{i=1}^{k-R} E[X_{n-R:i} |R]\Bigr] + (n-k)E\Bigl[E[X_{n-R:k-R} |R]\Bigr] \\
    &\quad - \lambda(n-k)q^k. \longalignedtag
  \end{longaligned}
  We expand to find the term
  \begin{longaligned}
    & E\Bigl[\sum_{i=1}^{k-R} E[X_{n-R:i} |R]\Bigr] \\
    &= E\Bigl[\sum_{i=1}^{k-R} \lambda\frac{\Gamma(n-R+1)}{\Gamma(n-R+1-1/\alpha)}\frac{\Gamma(n-R-i+1-1/\alpha)}{\Gamma(n-R-i+1)}\Bigr] \\
    &\stackrel{(a)}{=} E\Bigl[\lambda\frac{\Gamma(n-R+1)}{\Gamma(n-R+1-1/\alpha)} \sum_{j=n-k+1}^{n-R} \frac{\Gamma(j-1/\alpha)}{\Gamma(j)}\Bigr] \\
    &= E\Bigl[\lambda\frac{\Gamma(n-R+1)}{\Gamma(n-R+1-1/\alpha)} \\
    &\qquad\quad \times \Bigl(\sum_{j=0}^{n-R} \frac{\Gamma(j-1/\alpha)}{\Gamma(j)} - \sum_{j=0}^{n-k} \frac{\Gamma(j-1/\alpha)}{\Gamma(j)}\Bigr)\Bigr] \\
    &\stackrel{(b)}{=} E\Bigl[\lambda\frac{\Gamma(n-R+1)}{\Gamma(n-R+1-1/\alpha)} \frac{\alpha}{\alpha-1} \\
    &\qquad\quad \times \Bigl(\frac{\Gamma(n-R+1-1/\alpha)}{\Gamma(n-R)} - \frac{\Gamma(n-k+1-1/\alpha)}{\Gamma(n-k)}\Bigr)\Bigr] \\
    &= \frac{\alpha}{\alpha-1}\lambda(n-kq) \\
    &\quad - \frac{\alpha}{\alpha-1}\lambda\frac{\Gamma(n-k+1-1/\alpha)}{\Gamma(n-k)}E\Bigl[\frac{\Gamma(n-R+1)}{\Gamma(n-R+1-1/\alpha)}\Bigr].
  \end{longaligned}
  where $(a)$ is by defining $j=n-R-i+1$. $(b)$ is by Lemma \ref{lm_sum_gamma_ratios}. We also have
  \begin{longaligned}
    E\Bigl[ & E[X_{n-R:k-R} | R]\Bigr] \\
    &= \lambda\frac{\Gamma(n-k+1-1/\alpha)}{\Gamma(n-k+1)}E\Bigl[\frac{\Gamma(n-R+1)}{\Gamma(n-R+1-1/\alpha)}\Bigr].
  \end{longaligned}
  Substituting these in \eqref{eqn:eq_k_nd_wrelaunch_ECwcancel_lawoftotal} gives
  \begin{longaligned}
    & E[C^c] = kqE[X|X \leq \Delta] + k(1-q)\Delta \\
    &\quad + E\Bigl[\sum_{i=1}^{k-R} E[X_{n-R:i} |R]\Bigr] + (n-k)E\Bigl[E[X_{n-R:k-R} |R]\Bigr] \\
    &\quad - \lambda(n-k)q^k \\
    &= \frac{\alpha}{\alpha-1}k(\lambda-\Delta(1-q)) + k(1-q)\Delta \\
    &\quad - \lambda(n-k)q^k + \frac{\alpha}{\alpha-1}\lambda(n-kq) \\
    &\quad - \frac{\alpha}{\alpha-1}\lambda\frac{\Gamma(n-k+1-1/\alpha)}{\Gamma(n-k)}E[\frac{\Gamma(n-R+1)}{\Gamma(n-R+1-1/\alpha)}] \\
    &\quad + (n-k)\lambda\frac{\Gamma(n-k+1-1/\alpha)}{\Gamma(n-k+1)}E\Bigl[\frac{\Gamma(n-R+1)}{\Gamma(n-R+1-1/\alpha)}\Bigr] \\
    &= \frac{\alpha}{\alpha-1}(k(1-q)(\lambda-\Delta) + n\lambda) + k(1-q)\Delta - \lambda(n-k)q^k \\
    &\quad - \frac{\lambda}{\alpha-1}\frac{\Gamma(n-k+1-1/\alpha)}{\Gamma(n-k)}E\Bigl[\frac{\Gamma(n-R+1)}{\Gamma(n-R+1-1/\alpha)}\Bigr].
  \end{longaligned}
  
  In the proof of Thm.~\ref{thm_k_nd_wrelaunch_ET__EC}, we showed that
  \begin{longaligned}
    \frac{\Gamma(n-k+1-1/\alpha)}{\Gamma(n-k+1)} & E\Bigl[\frac{\Gamma(n-R+1)}{\Gamma(n-R+1-1/\alpha)}\Bigr] \\
    &\approx \frac{B(n-kq+1, -1/\alpha)}{B(n-k+1, -1/\alpha)}.
  \end{longaligned}
  Using which we can finalize the proof as
  \begin{longaligned}
    E[C^c] &= \frac{\alpha}{\alpha-1}(k(1-q)(\lambda-\Delta) + n\lambda) + k(1-q)\Delta \\
    &\quad - \lambda(n-k)q^k - \frac{\lambda}{\alpha-1}(n-k)\frac{B(n-kq+1, -1/\alpha)}{B(n-k+1, -1/\alpha)}.
  \end{longaligned}
\end{proof}


==> proofs/proof_of_k_wrelaunch_T_C.tex <==
\begin{proof}
  % ### Pr{T > t} ### %
  Let $T_{wo}$ be the latency of executing a job of $k$ tasks with no redundancy and no straggler relaunch. Let $R \sim \textit{Bin}(k, q)$ be the number of tasks completed before time $\Delta$ where $q = \mathbbm{1}(\Delta > \lambda)(1 - (\lambda/\Delta)^{\alpha})$. By the law of total probability
  \begin{longaligned}
    & Pr\{T_{wo} > t\} = Pr\{T_{wo} > t|R=k\}Pr\{R=k\} \\
    &\quad + \sum_{r=0}^{k-1} Pr\{T_{wo} > t|R=r\}Pr\{R=r\} \\
    &= Pr\{X_{k:k} > t|R=k\}Pr\{R=k\} \\
    &\quad + \sum_{r=0}^{k-1} Pr\{(X|X > \Delta)_{k-r:k-r} > t|R=r\}Pr\{R=r\}.
  \end{longaligned}
  Repeating the same for $T$
  \begin{longaligned}
    Pr\{T > t\} &= Pr\{T > t|R=k\}Pr\{R=k\} \\
    &\quad + \sum_{r=0}^{k-1} Pr\{T > t|R=r\}Pr\{R=r\} \\
    &= Pr\{X_{k:k} > t|R=k\}Pr\{R=k\} \\
    &\quad + \sum_{r=0}^{k-1} Pr\{X_{k-r:k-r} + \Delta > t\}Pr\{R=r\} \\
    &= Pr\{X_{k:k} > t\} = 1 - Pr\{X_{k:k} \leq t\} \\
    &= 1 - \bigl[\mathbbm{1}(t > \lambda)(1 - (\lambda/t)^{\alpha})\bigr]^k.
  \end{longaligned}
  Then
  \begin{longaligned}
    & Pr\{T > t\} - Pr\{T_{wo} > t\} \\
    &= \sum_{r=0}^{k-1} \Bigl[Pr\{X_{k-r:k-r} > t-\Delta\} \\
    &\qquad\quad - Pr\{(X|X > \Delta)_{k-r:k-r} > t\}\Bigr] Pr\{R=r\} \\
    &= \sum_{r=0}^{k-1} \Bigl[Pr\{(X|X > \Delta)_{k-r:k-r} \leq t\} \\
    &\qquad\quad - Pr\{X_{k-r:k-r} \leq t-\Delta\}\Bigr]Pr\{R=r\} \\
    &= \sum_{r=0}^{k-1} \Bigl[Pr\{X \leq t|X > \Delta\}^{k-r} \\
    &\qquad\quad - Pr\{X \leq t-\Delta\}^{k-r}\Bigr]Pr\{R=r\} \\
    &= E\bigl[Pr\{X \leq t|X > \Delta\}^{k-R}\bigr] - E\bigl[Pr\{X \leq t-\Delta\}^{k-R}\bigr] \\
    &= \bigl[q + Pr\{X \leq t|X > \Delta\}(1-q) \bigr]^k \\
    &\quad - \bigl[q + Pr\{X \leq t-\Delta\}(1-q) \bigr]^k \\
    &= \bigl[q + \mathbbm{1}(t > \Delta)\bigl(1 - (\Delta/t)^{\alpha} \bigr)(1-q) \bigr]^k \\
    &\quad - \bigl[q + \mathbbm{1}(t > \Delta+\lambda)\bigl(1 - (\lambda/(t-\Delta))^{\alpha} \bigr)(1-q) \bigr]^k.
  \end{longaligned}
  Tail distribution of the job execution time as given in \eqref{eqn:eq_k_wrelaunch_tail__ET} follows by noticing that $T_{wo} \sim X_{k:k}$, from which $Pr\{T_{wo} > t\}$ is easily obtained.
  
  % ### E[T] ### %
  Next we derive the latency. Using the law of total expectation
  \begin{longaligned}
    E[T] &= E[T|T \leq \Delta]Pr\{T \leq \Delta\} + E[T|T > \Delta]Pr\{T > \Delta\} \\
    &= E[X_{k:k}|X_{k:k} \leq \Delta]Pr\{X_{k:k} \leq \Delta\} \\
    &\quad + E[T|X_{k:k} > \Delta]Pr\{X_{k:k} > \Delta\} \\
    &\stackrel{(a)}{=} E[X_{k:k}|X_{k:k} \leq \Delta]Pr\{X_{k:k} \leq \Delta\} \\
    &\quad + \sum_{r=0}^{k-1} E[\Delta + X_{k-r:k-r}]Pr\{R=r\}.
  \end{longaligned}
  where $(a)$ is by noticing that given $R=r$, the residual lifetime of the job after $\Delta$ is $X_{k-r:k-r}$. Similar observation can be made for $T_{wo}$ but tasks are not relaunched in this case, given $R=r$, the residual lifetime of the job after $\Delta$ is $(X-\Delta|X > \Delta)_{k-r:k-r}$. Using this observation
  \begin{longaligned}
    E[T_{wo}] &= E[T_{wo}|T_{wo} \leq \Delta]Pr\{T_{wo} \leq \Delta\} \\
    &\quad + E[T_{wo}|T_{wo} > \Delta]Pr\{T_{wo} > \Delta\} \\
    &= E[X_{k:k}|X_{k:k} \leq \Delta]Pr\{X_{k:k} \leq \Delta\} \\
    &\quad + E[T|X_{k:k} > \Delta]Pr\{X_{k:k} > \Delta\} \\
    &= E[X_{k:k}|X_{k:k} \leq \Delta]Pr\{X_{k:k} \leq \Delta\} \\
    &\quad + \sum_{r=0}^{k-1} E[\Delta + (X-\Delta|X > \Delta)_{k-r:k-r}]Pr\{R=r\}.
  \end{longaligned}
  Taking the difference
  \begin{longaligned}[\label{eqn:eq_k_wrelaunch_ET_diff}]
    & E[T - T_{wo}] \\
    &= \sum_{r=0}^{k-1} E\bigl[X_{k-r:k-r} - (X-\Delta|X > \Delta)_{k-r:k-r}\bigr]Pr\{R=r\} \\
    &\stackrel{(a)}{=} \sum_{r=0}^{k-1} \Bigl[(k-r)\int_0^1 \bigl(F^{-1}(u) - \tilde{F}^{-1}(u)\bigr)u^{k-r-1} du \Bigr]Pr\{R=r\}. \longalignedtag
  \end{longaligned}
  where $(a)$ is by the definition of order statistics where $\tilde{F}(x) = Pr\{X-\Delta=x|X > \Delta\}$. One can find $\tilde{F}^{-1}(x) = F^{-1}\bigl(1-(1-x)F_c(\Delta)\bigr) - \Delta$ which is equal to $\lambda(1-x)^{-1/\alpha}$ for $X \sim \textit{Pareto}(\lambda, \alpha)$. Then, we find $D_{\Delta}(u) = F^{-1}(u) - \tilde{F}^{-1}(u)$ as
  \begin{longaligned}
    D_{\Delta}(u) =
    \begin{cases}
      \Delta & \Delta \leq \lambda, \\
      (\lambda-\Delta)(1-u)^{-1/\alpha} + \Delta & o.w.
    \end{cases}
  \end{longaligned}
  substituting which firstly for $\Delta \leq \lambda$, we have
  \begin{longaligned}[\label{eqn:eq_k_wrelaunch_ET_diff_inner_d_leq_loc}]
    & E\bigl[X_{k-r:k-r} - (X-\Delta|X > \Delta)_{k-r:k-r}\bigr] \\
    &= (k-r)\int_0^1 \Delta u^{k-r-1} du = \Delta (k-r) B(k-r, 1) = \Delta. \longalignedtag
  \end{longaligned}
  and secondly for $\Delta > \lambda$, we have
  \begin{longaligned}[\label{eqn:eq_k_wrelaunch_ET_diff_inner_d_g_loc}]
    & E[X_{k-r:k-r} - (X-\Delta|X > \Delta)_{k-r:k-r}] \\
    &= (k-r) \int_0^1 \bigl[\Delta + (\lambda-\Delta)(1-u)^{-1/\alpha}\bigr] u^{k-r-1} du \\
    &= (k-r)\Delta\int_0^1 u^{k-r-1} du \\
    &\quad + (k-r)(\lambda-\Delta) \int_0^1 u^{k-r-1}(1-u)^{-1/\alpha} du \\
    &= \Delta + (k-r)(\lambda-\Delta)B(k-r, 1-1/\alpha) \\
    &= \Delta + (\lambda-\Delta)\frac{\Gamma(1-1/\alpha)}{\Gamma(k-r+1-1/\alpha)} (k-r)!. \longalignedtag
  \end{longaligned}
  Firstly substituting \eqref{eqn:eq_k_wrelaunch_ET_diff_inner_d_leq_loc} in \eqref{eqn:eq_k_wrelaunch_ET_diff} for $\Delta \leq \lambda$
  \begin{longaligned}[\label{eqn:eq_k_wrelaunch_ET_diff_d_leq_loc}]
    E[T - T_{wo}] &= \sum_{r=0}^{k-1} \Delta Pr\{R=r\} \\
    &= \Delta I(1-q;1,k) \stackrel{(a)}{=} \Delta. \longalignedtag
  \end{longaligned}
  where last equality is by using $q = 0$ for $\Delta \leq \lambda$. 
  
  Secondly substituting \eqref{eqn:eq_k_wrelaunch_ET_diff_inner_d_g_loc} in \eqref{eqn:eq_k_wrelaunch_ET_diff} for $\Delta > \lambda$
  \begin{longaligned}[\label{eqn:eq_k_wrelaunch_ET_diff_d_g_loc}]
    & E[T - T_{wo}] \\
    &= \sum_{r=0}^{k-1} \Bigl[\Delta + (\lambda-\Delta)\frac{\Gamma(1-1/\alpha)(k-r)!}{\Gamma(k-r+1-1/\alpha)} \Bigr] Pr\{R=r\} \\
    &= \Delta I(1-q;1,k) \\
    &\quad + (\lambda-\Delta)\Gamma(1-1/\alpha) \sum_{r=0}^{k-1} \frac{(k-r)!k! q^r (1-q)^{k-r}}{\Gamma(k-r+1-1/\alpha)r!} \\
    &= \Delta I(1-q;1,k) \\
    &\quad + \frac{(\lambda-\Delta)\Gamma(1-1/\alpha) (1-q)^{1/\alpha} k!}{(k-1/\alpha)!} \\
    &\quad\quad \times \sum_{r=0}^{k-1} \binom{k-1/\alpha}{r} q^r (1-q)^{k-1/\alpha-r} \\
    &= \Delta I(1-q;1,k) \\
    &\quad + (\lambda-\Delta)\Gamma(1-1/\alpha) \frac{\lambda}{\Delta}\frac{k!}{(k-1/\alpha)!} I(1-q;1-1/\alpha,k). \longalignedtag
  \end{longaligned}
  Finally it is easy to find,
  \begin{longaligned}
    E[T_{wo}] = E[X_{k:k}] = \lambda k!\frac{\Gamma(1-1/\alpha)}{\Gamma(k+1-1/\alpha)}
  \end{longaligned}
  using which together with \eqref{eqn:eq_k_wrelaunch_ET_diff}, \eqref{eqn:eq_k_wrelaunch_ET_diff_d_leq_loc}
and \eqref{eqn:eq_k_wrelaunch_ET_diff_d_g_loc} shows yields the latency as given in \eqref{eqn:eq_k_wrelaunch_tail__ET}.
  
  % ### E[C], E[C^c] ### %
  Expressions given in \eqref{eqn:eq_k_wrelaunch_EC} for cost with and without task cancellation can be found by substituting $c=0$ in the expressions given in Thm.~\ref{thm_k_cn_wrelaunch_ET}.
\end{proof}

